Ad-hoc polymorphic delimited continuations

We designed and implemented a framework for creating extensible domain-specific languages that consists of library-defined keywords. First-class language features in other programming languages can be implemented as libraries with the help of our framework. The core concept in our framework is the type class Dsl, which can be considered as both the ad-hoc polymorphic version of a delimited continuation and a more generic version of Monad. Thus it can be also used as a statically typed extensible effect system that is more efficient and more concise than existing Monad-based effect systems.

==> latexmkrc <==
@default_files = ('paper.tex');

add_cus_dep( 'glo', 'gls', 0, 'makeglo2gls' );

sub makeglo2gls {
    system("makeindex -l -s \"$_[0].ist\" -t \"$_[0].glg\" -o \"$_[0].gls\" \"$_[0].glo\"" );
}

$latex = 'latex  %O  --shell-escape %S';
$pdflatex = 'pdflatex  %O  --shell-escape %S';
$pdf_mode = 1;

==> paper-dot2tex-fig1.tex <==

\begin{tikzpicture}[>=latex,line join=bevel,scale=0.78,transform shape]
%%
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (0.0bp,8.0bp) -- (0.0bp,199.0bp) -- (181.25bp,199.0bp) -- (181.25bp,8.0bp) -- cycle;
  \draw (90.623bp,182.5bp) node {$\textrm{a code block that returns an \lstinline{Eff}}$};
\end{scope}
  \node (Effect_0) at (90.623bp,147.0bp) [draw,ellipse] {$Effect_0$};
  \node (Effect_1) at (90.623bp,107.0bp) [draw,ellipse] {$Effect_1$};
  \node (Effect_dots) at (90.623bp,67.0bp) [draw,draw=none] {${\vdots}$};
  \node (Effect_n) at (90.623bp,27.0bp) [draw,ellipse] {$Effect_n$};
  \node (Eff) at (301.16bp,84.0bp) [draw,ellipse] {$Eff$};
  \node (Handler_0) at (461.55bp,147.0bp) [draw,ellipse] {$Handler_0$};
  \node (Handler_1) at (461.55bp,106.0bp) [draw,ellipse] {$Handler_1$};
  \node (Handler_dots) at (461.55bp,66.0bp) [draw,draw=none] {${\vdots}$};
  \node (Handler_n) at (461.55bp,26.0bp) [draw,ellipse] {$Handler_n$};
  \draw [->] (Effect_0) ..controls (157.87bp,146.89bp) and (218.42bp,142.08bp)  .. (264.25bp,119.0bp) .. controls (272.16bp,115.01bp) and (279.45bp,108.67bp)  .. (Eff);
  \draw (227.75bp,151.0bp) node {$\textrm{interpreted by}$};
  \draw (128.01bp,141.49bp) node {$$};
  \draw (286.52bp,100.34bp) node {$$};
  \draw [->] (Effect_1) ..controls (160.45bp,99.409bp) and (231.65bp,91.556bp)  .. (Eff);
  \draw (227.75bp,105.0bp) node {$\textrm{interpreted by}$};
  \draw (126.62bp,97.802bp) node {$$};
  \draw (276.15bp,79.986bp) node {$$};
  \draw [->] (Effect_n) ..controls (158.29bp,25.759bp) and (218.27bp,29.319bp)  .. (264.25bp,51.0bp) .. controls (271.93bp,54.625bp) and (279.12bp,60.481bp)  .. (Eff);
  \draw (227.75bp,61.0bp) node {$\textrm{interpreted by}$};
  \draw (128.49bp,19.873bp) node {$$};
  \draw (286.16bp,67.878bp) node {$$};
  \draw [->] (Eff) ..controls (315.62bp,103.16bp) and (326.02bp,115.29bp)  .. (338.08bp,122.0bp) .. controls (361.85bp,135.22bp) and (391.69bp,141.48bp)  .. (Handler_0);
  \draw (373.08bp,152.0bp) node {$\textrm{dispatched to}$};
  \draw (315.16bp,100.4bp) node {$$};
  \draw (420.69bp,139.58bp) node {$$};
  \draw [->] (Eff) ..controls (343.69bp,89.768bp) and (386.18bp,95.67bp)  .. (Handler_1);
  \draw (373.08bp,108.0bp) node {$\textrm{dispatched to}$};
  \draw (326.02bp,80.481bp) node {$$};
  \draw (423.13bp,95.636bp) node {$$};
  \draw [->] (Eff) ..controls (316.03bp,65.445bp) and (326.35bp,54.14bp)  .. (338.08bp,48.0bp) .. controls (361.63bp,35.677bp) and (390.82bp,30.117bp)  .. (Handler_n);
  \draw (373.08bp,58.0bp) node {$\textrm{dispatched to}$};
  \draw (315.5bp,67.753bp) node {$$};
  \draw (419.76bp,20.721bp) node {$$};
%
\end{tikzpicture}


==> paper-dot2tex-fig2.tex <==

\begin{tikzpicture}[>=latex,line join=bevel,transform shape]
%%
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (0.0bp,8.0bp) -- (0.0bp,201.0bp) -- (205.78bp,201.0bp) -- (205.78bp,8.0bp) -- cycle;
  \draw (102.89bp,183.5bp) node {$\textrm{a code block that returns any \texttt{Domain}}$};
\end{scope}
  \node (Keyword_0) at (102.89bp,147.0bp) [draw,ellipse] {$Keyword_0$};
  \node (Keyword_1) at (102.89bp,107.0bp) [draw,ellipse] {$Keyword_1$};
  \node (Keyword_dots) at (102.89bp,67.0bp) [draw,draw=none] {${\vdots}$};
  \node (Keyword_n) at (102.89bp,27.0bp) [draw,ellipse] {$Keyword_n$};
  \node (Dsl_0) at (325.95bp,150.0bp) [draw,ellipse] {$Dsl_0$};
  \node (Dsl_1) at (325.95bp,107.0bp) [draw,ellipse] {$Dsl_1$};
  \node (Dsl_dots) at (325.95bp,67.0bp) [draw,draw=none] {${\vdots}$};
  \node (Dsl_n) at (325.95bp,27.0bp) [draw,ellipse] {$Dsl_n$};
  \draw [->] (Keyword_0) ..controls (183.7bp,148.08bp) and (255.06bp,149.05bp)  .. (Dsl_0);
  \draw (251.28bp,159.0bp) node {$\textrm{interpreted by}$};
  \draw (146.39bp,141.5bp) node {$$};
  \draw (300.09bp,143.74bp) node {$$};
  \draw [->] (Keyword_1) ..controls (183.7bp,107.0bp) and (255.06bp,107.0bp)  .. (Dsl_1);
  \draw (251.28bp,117.0bp) node {$\textrm{interpreted by}$};
  \draw (146.39bp,101.0bp) node {$$};
  \draw (300.09bp,101.0bp) node {$$};
  \draw [->] (Keyword_n) ..controls (183.96bp,27.0bp) and (254.29bp,27.0bp)  .. (Dsl_n);
  \draw (251.28bp,37.0bp) node {$\textrm{interpreted by}$};
  \draw (146.89bp,21.0bp) node {$$};
  \draw (299.32bp,21.0bp) node {$$};
%
\end{tikzpicture}

